Late-Time Supernovae Radio Re-brightening in the VAST Pilot Survey

We present our analysis of supernovae serendipitously found to be radio-bright several years after their optical discovery. We used recent observations from the Australian SKA Pathfinder taken as part of the pilot Variables and Slow Transients and Rapid ASKAP Continuum Survey programs. We identified 29 objects by cross-matching sources from these ASKAP observations with known core-collapse supernovae below a declination of $+40^{\circ}$ and with a redshift of $z\leq0.15$. Our results focus on eight cases that show potential late-time radio emission. These supernovae exhibit significantly greater amounts of radio emission than expected from the standard model of a single shockwave propagating through a spherical circumstellar medium, with a constant density structure produced by regular stellar mass-loss. We also discuss how we can learn from future ASKAP surveys about the circumstellar environments and emission mechanisms of supernovae that undergo late-time radio re-brightening. This pilot work tested and confirmed the potential of the Variables and Slow Transients survey to discover and study late-time supernova emission.

==> tables/RISS_results.tex <==
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
    RA & Dec & H$_{\alpha}$ & eH$_{\alpha}$ & $\xi$ & e$\xi$ & $sm$ & e $sm$ & $m$ & e$m$ & $t_0$ & e$t_0$ & RMS$_{1yr}$ & eRMS$_{1yr}$ & $\theta_r$ & e$\theta_r$ & $\nu_0$ & $f_0$ \\ \hline
    14:22:22.7 & $+$00:23:23 & 0.4207763671875 & 0.275390625 & 335.38214459033696 & 131.70098544906983 & 8.551405335310847e-05 & 5.5967426305869594e-05 & 0.14393067236171025 & 0.018840012497324615 & 43.28600242400552 & 16.997950747663637 & 0.003325108910539849 & 0.01888520622426419 & 2.5364336408983945e-08 & 5.706833690055646e-07 & 27.150642622128025 & 7.562817077741719e-11 \\ 
    04:10:59.4 & $-$31:24:49 & 1.2958984375 & 1.328125 & 658.645528671846 & 405.0149106069336 & 0.00026336443261243403 & 0.0002699138130992651 & 0.11493423707894093 & 0.023558488711457725 & 85.00790042199331 & 52.27313583943021 & 0.0013520418279758506 & 0.023573154526437483 & 4.9812154401251973e-08 & 1.755000312186894e-06 & 40.383020289291196 & 7.562817077741719e-11 \\ 
    16:21:48.9 & $-$02:16:17 & 0.66162109375 & 0.30078125 & 440.02241512334706 & 120.02382027324815 & 0.00013446074444800615 & 6.112753908382729e-05 & 0.13147456216458178 & 0.011953996491536523 & 56.79136959098192 & 15.490840699442264 & 0.002315044752600209 & 0.011970663524637335 & 3.3278087840926673e-08 & 5.200841428631975e-07 & 31.8532334391649 & 7.562817077741719e-11 \\
    05:00:13.7 & $-$03:20:50 & 0.728759765625 & 0.3125 & 466.29403110866286 & 119.9711263169109 & 0.00014810530410613865 & 6.350914190988988e-05 & 0.12895753248053285 & 0.011059674358941 & 60.18210833949813 & 15.48403976874713 & 0.0021427885469392357 & 0.011073406887613046 & 3.5264964282077926e-08 & 5.198558596930525e-07 & 32.95856356495504 & 7.562817077741719e-11 \\
    21:18:50.7 & $-$57:38:42 & 0.609619140625 & 1.2578125 & 418.93275101794524 & 518.6243276874025 & 0.00012389243056531996 & 0.0002556242689024657 & 0.13364474769895518 & 0.055149199369036804 & 54.06943800841971 & 66.93610338989986 & 0.002471724371874255 & 0.05523402247210196 & 3.168311479839758e-08 & 2.2472895579994656e-06 & 30.946119145682626 & 7.562817077741719e-11 \\
    18:25:02.1 & $+$27:31:53 & 1.033203125 & 0.34375 & 574.9374485285014 & 114.77012351758277 & 0.00020997709361836314 & 6.986004882492125e-05 & 0.12026145877868835 & 0.008002274864138561 & 74.20414053662563 & 14.812773801222326 & 0.0016206839390495976 & 0.008008812072753356 & 4.3481467315587e-08 & 4.973189788870513e-07 & 37.279889258651544 & 7.562817077741719e-11 \\ 
    21:59:04.1 & $+$18:11:11 & 0.9287109375 & 0.326171875 & 539.3088168809007 & 113.64615287316668 & 0.00018874122179113328 & 6.62876627757214e-05 & 0.12285348854257201 & 0.00862945675581532 & 69.60574118610018 & 14.667708845250583 & 0.0017649907385384623 & 0.008637468079881102 & 4.078693649489651e-08 & 4.924486347590573e-07 & 35.903071505734836 & 7.562817077741719e-11 \\ 
    2:35:30.2 & $-$09:21:14 & 0.505126953125 & 0.296875 & 374.23939609666047 & 131.969584568476 & 0.00010265656601404771 & 6.0333681176416576e-05 & 0.1387661370967341 & 0.016311225431130394 & 48.30110269103796 & 17.032617417673464 & 0.00287293931950919 & 0.016342657051667524 & 2.8303038135391034e-08 & 5.718472380067396e-07 & 28.959144768847285 & 7.562817077741719e-11 \\ \hline
\end{tabular}

